Euclid: Supercharging Multimodal LLMs with Synthetic High-Fidelity Visual Descriptions

Multimodal large language models (MLLMs) have made rapid progress in recent years, yet continue to struggle with low-level visual perception (LLVP) -- particularly the ability to accurately describe the geometric details of an image. This capability is crucial for applications in areas such as robotics, medical image analysis, and manufacturing. In this paper, we first introduce Geoperception, a benchmark designed to evaluate an MLLM's ability to accurately transcribe 2D geometric information from an image. Using this benchmark, we demonstrate the limitations of leading MLLMs, and then conduct a comprehensive empirical study to explore strategies for improving their performance on geometric tasks. Our findings highlight the benefits of certain model architectures, training techniques, and data strategies, including the use of high-fidelity synthetic data and multi-stage training with a data curriculum. Notably, we find that a data curriculum enables models to learn challenging geometry understanding tasks which they fail to learn from scratch. Leveraging these insights, we develop Euclid, a family of models specifically optimized for strong low-level geometric perception. Although purely trained on synthetic multimodal data, Euclid shows strong generalization ability to novel geometry shapes. For instance, Euclid outperforms the best closed-source model, Gemini-1.5-Pro, by up to 58.56% on certain Geoperception benchmark tasks and 10.65% on average across all tasks.

==> sections/result.tex <==
\section{Evaluation Results, Analysis and Discussion.}

\input{tabs/euclid_eval}

We evaluate \euclid{} on the four task in Geoperception that \euclid{} is adapted on, the result is shown in~\cref{tab:euclid_performance}. Although only trained on several very simple synthetic geometry shapes, \euclid{} outperform all current leading MLLMs greatly, showing great generalize ability on real world geometry shapes. Specifically, on the most challenging task for current leading MLLMs,~\texttt{PointLiesOnLine}, ~\euclid{} reaches at most 78.94\% accuracy, which is almost three times better than gemini-pro. 

We also train~\euclid{} on the mixture of four tasks. During training, the dataset between each tasks are equally divided and 

\jiarui{Paragraph: Test result on Geoperception, with enough training data and proper training strategy, a very small model can easily beat even the best leading MLLMs on geometry perception tasks.}

\jiarui{Paragraph: Adapt the model after geometry training to a new task.}
